Ground state energy and magnetization curve of a frustrated magnetic system from real-time evolution on a digital quantum processor

Models of interacting many-body quantum systems that may realize new exotic phases of matter, notably quantum spin liquids, are challenging to study using even state-of-the-art classical methods such as tensor network simulations. Quantum computing provides a promising route for overcoming these difficulties to find ground states, dynamics, and more. In this paper, we argue that recently developed hybrid quantum-classical algorithms based on real-time evolution are promising methods for solving a particularly important model in the search for spin liquids, the antiferromagnetic Heisenberg model on the two-dimensional kagome lattice. We show how to construct efficient quantum circuits to implement time evolution for the model and to evaluate key observables on the quantum computer, and we argue that the method has favorable scaling with increasing system size. We then restrict to a 12-spin star plaquette from the kagome lattice and a related 8-spin system, and we give an empirical demonstration on these small systems that the hybrid algorithms can efficiently find the ground state energy and the magnetization curve. For these demonstrations, we use four levels of approximation: exact state vectors, exact state vectors with statistical noise from sampling, noisy classical emulators, and (for the 8-spin system only) real quantum hardware, specifically the Quantinuum H1-1 processor; for the noisy simulations and hardware demonstration, we also employ error mitigation strategies based on the symmetries of the Hamiltonian. Our results strongly suggest that these hybrid algorithms present a promising direction for studying quantum spin liquids and more generally for resolving important unsolved problems in condensed matter theory and beyond.

==> circuit_diagrams/Trotter_parallelization_tikz.tex <==
\begin{tikzcd}[ampersand replacement=\&, row sep={0.4cm,between origins}, column sep=0.1cm]
\lstick{0}  \& \qw\& \ctrl{1}\gategroup[3,steps=8,style={rounded corners, inner sep=-0.5pt}]{} \& \ctrl{2} \& \qw \& \ctrl{1} \& \ctrl{1} \& \ctrl{2} \& \qw \& \ctrl{1} \& \qw  \& \qw
\& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw\\
\lstick{1}  \& \qw\& \targ{}  \& \qw \& \ctrl{1} \& \targ{}  \& \targ{}  \& \qw \& \ctrl{1} \& \targ{}  \& \qw \& \qw
\& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw\\
\lstick{2}  \& \qw\& \qw \& \targ{}  \& \targ{}  \& \qw      \& \qw \& \targ{}  \& \targ{}  \& \qw \& \qw \& \qw
\& \ctrl{1}\gategroup[3,steps=8,style={rounded corners, inner sep=-0.5pt}]{} \& \ctrl{2} \& \qw \& \ctrl{1} \& \ctrl{1} \& \ctrl{2} \& \qw \& \ctrl{1} \& \qw \& \qw\\
%
\lstick{3}  \& \qw\& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw
\& \targ{}  \& \qw \& \ctrl{1} \& \targ{}  \& \targ{}  \& \qw \& \ctrl{1} \& \targ{} \& \qw \& \qw\\
%
\lstick{4}  \& \qw\& \ctrl{1}\gategroup[3,steps=8,style={rounded corners, inner sep=-0.5pt}]{} \& \ctrl{2} \& \qw \& \ctrl{1} \& \ctrl{1} \& \ctrl{2} \& \qw \& \ctrl{1} \& \qw \& \qw
\& \qw \& \targ{}  \& \targ{}  \& \qw      \& \qw \& \targ{}  \& \targ{}  \& \qw \& \qw \& \qw\\
\lstick{5}  \& \qw\& \targ{}  \& \qw \& \ctrl{1} \& \targ{}  \& \targ{}  \& \qw \& \ctrl{1} \& \targ{}\& \qw \& \qw
\& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw\\
\lstick{6}  \& \qw\& \qw \& \targ{}  \& \targ{}  \& \qw      \& \qw \& \targ{}  \& \targ{}  \& \qw \& \qw \& \qw
\& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw
\end{tikzcd}
\begin{huge}
    $\rightarrow$
\end{huge}
\begin{tikzcd}[ampersand replacement=\&, row sep={0.4cm,between origins}, column sep=0.1cm]
\lstick{0}  \& \qw\& \ctrl{1}\gategroup[3,steps=8,style={rounded corners, inner sep=-0.5pt}]{} \& \ctrl{2} \& \qw \& \ctrl{1} \& \ctrl{1} \& \ctrl{2} \& \qw \& \ctrl{1} \& \qw  \& \qw
\& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw\\
\lstick{1}  \& \qw\& \targ{}  \& \qw \& \ctrl{1} \& \targ{}  \& \targ{}  \& \qw \& \ctrl{1} \& \targ{}  \& \qw \& \qw
\& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw\\
\lstick{2}  \& \qw\& \qw \& \targ{}  \& \targ{}  \& \qw      \& \qw \& \targ{}  \& \targ{}  \& \qw \& \qw \& \qw
\& \ctrl{1}\gategroup[3,steps=8,style={rounded corners, inner sep=-0.5pt}]{} \& \ctrl{2} \& \qw \& \ctrl{1} \& \ctrl{1} \& \ctrl{2} \& \qw \& \ctrl{1} \& \qw \& \qw\\
%
\lstick{3}  \& \qw\& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw
\& \targ{}  \& \qw \& \ctrl{1} \& \targ{}  \& \targ{}  \& \qw \& \ctrl{1} \& \targ{} \& \qw \& \qw\\
%
\lstick{4}  \& \qw\& \ctrl{1}\gategroup[3,steps=8,style={rounded corners, inner sep=-0.5pt}]{} \& \ctrl{2} \& \qw \& \ctrl{1} \& \ctrl{1} \& \ctrl{2} \& \qw \& \ctrl{1} \& \qw \& \qw
\& \qw \& \targ{}  \& \targ{}  \& \qw      \& \qw \& \targ{}  \& \targ{}  \& \qw \& \qw \& \qw\\
\lstick{5}  \& \qw\& \targ{}  \& \qw \& \ctrl{1} \& \targ{}  \& \targ{}  \& \qw \& \ctrl{1} \& \targ{}\& \qw \& \qw
\& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw\\
\lstick{6}  \& \qw\& \qw \& \targ{}  \& \targ{}  \& \qw      \& \qw \& \targ{}  \& \targ{}  \& \qw \& \qw \& \qw
\& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw \& \qw
\end{tikzcd}
